From dot to ring: the role of friction on the deposition pattern of a drying colloidal suspension droplet

The deposition of particles on a substrate by drying a colloidal suspension droplet is at the core of applications ranging from traditional printing on paper to printable electronics or photovoltaic devices. The self-pinning induced by the accumulation of particles at the contact line plays an important role in the formation of the deposition. In this paper, we investigate both numerically and theoretically, the effect of friction between the particles and the substrate on the deposition pattern. Without friction, the contact line shows a stick-slip behaviour and a dot-like deposit is left after the droplet is evaporated. By increasing the friction force, we observe a transition from a dot-like to a ring-like deposit. We propose a theoretical model to predict the effective radius of the particle deposition as a function of the friction force. Our theoretical model predicts a critical friction force when the self-pinning happens and the effective radius of deposit increases with increasing friction force, confirmed by our simulation results. Our results can find implications for developing active control strategies for the deposition of drying droplets.

==> draw-drop-md.tex <==
\begin{figure}[htbp]
\centering
 \begin{tikzpicture}
	\fill[blue,opacity=0.2] (-4,0) rectangle (4.0,3.0);
% 	\fill[white,opacity=0.4] (-3,0) rectangle (3.0,3.0);
	
	% 1st janus
% 	\draw (0,-0.0) circle (0.8);
% 	\shade[ball color=yellow] (0,-0.0) circle (1.75);
	 \filldraw[fill=red!30!white, draw=green!50!black]
      %(0,0) -- (-1.0,-1.45) arc (235:415:1.75) -- (0,0);
      (0.0,0) -- (3.45,0.0) arc (20:160:3.7) -- (-0.0,0);
	
	\draw[ultra thick,black] (-4.0,0) to (4.0,0);
	\draw[ultra thick,black, dashed] (-4.0,0) to (-4.0,3);
	\draw[ultra thick,black, dashed] (4.0,0) to (4.0,3);
	\draw[ultra thick,black, dashed] (-4.0,3) to (4.0,3);
	%magnetic field
% 	\draw[ultra thick, black,arrows=->] (0.5,2.0) to (-0.5,2.0);
    
  	
%   	\draw[ultra thick, black] (-0.5,-0.72) -- (0.5,0.72); %  new add
%   	\draw[thick, black, dashed] (0.7,0.0) -- (0.7,0.5);  % new add 

%contact angle
  \draw[thick, black, dotted] (-3.5,0) to (-2.5,2);
  \draw[thick,black] (-3.0,0.0) to [out=120,in=90] (-3.3,0.4);
 \node at (-3.0,0.4) [fontscale=2] {$\theta$};
 

% xyz coordinates
 \draw[thick, black,arrows=->] (2,1) to (2,2);
 \node at (2.2,1.75) [fontscale=2] {z};
 \draw[thick, black,arrows=->] (2,1) to (3,1);
 \node at (2.5,1.2) [fontscale=2] {r};
  \draw[thick, black,arrows=->] (0,0) to (0,2.45);
 \node at (0.2,1.0) [fontscale=2] {h};
  \draw[thick, black,arrows=->] (0,0.2) to (3.45,0.2);
   \draw[thick, black,arrows=->] (3.45,0.2) to (0,0.2);
   \draw[thick, black] (3.45,0.0) to (3.45,0.3);
 \node at (1.25,0.55) [fontscale=2] {$R_d$};
 %particles
%  \fill[black,opacity=0.7] (-2,0.4) circle (0.1);
 \shade[ball color=green] (-2,0.4) circle (0.1);
 \shade[ball color=green] (-2.6,0.3) circle (0.1);
  \shade[ball color=green] (-1.6,1.8) circle (0.1);
 \shade[ball color=green] (2,0.4) circle (0.1);
 \shade[ball color=green] (-1,0.8) circle (0.1);
 \shade[ball color=green] (1.3,0.9) circle (0.1);
  \shade[ball color=green] (0.3,2.2) circle (0.1);
  \shade[ball color=green] (1.3,2.0) circle (0.1);
 %substrate
  \fill[red,opacity=0.5] (-3.5,-0.4) rectangle (3.5,0.0);
  \fill[blue,opacity=0.5] (-4.0,-0.4) rectangle (-3.5,0.0);
  \fill[blue,opacity=0.5] (3.5,-0.4) rectangle (4.0,0.0);
  \draw[step=2mm, black] (-4.0,-0.4) grid (4.0,0.0);
\end{tikzpicture}


\caption{Sketch of a colloidal suspension droplet sitting on a substrate.
The droplet height is $h$ and the radius is $R_d$. 
The green dots represent colloidal particles.
In simulations, we apply evaporation boundary at the top and sizes of system (dashed line).
}
\label{fig:drop-geo}
\end{figure}
